Classification of Consumer Belief Statements From Social Media

Social media offer plenty of information to perform market research in order to meet the requirements of customers. One way how this research is conducted is that a domain expert gathers and categorizes user-generated content into a complex and fine-grained class structure. In many of such cases, little data meets complex annotations. It is not yet fully understood how this can be leveraged successfully for classification. We examine the classification accuracy of expert labels when used with a) many fine-grained classes and b) few abstract classes. For scenario b) we compare abstract class labels given by the domain expert as baseline and by automatic hierarchical clustering. We compare this to another baseline where the entire class structure is given by a completely unsupervised clustering approach. By doing so, this work can serve as an example of how complex expert annotations are potentially beneficial and can be utilized in the most optimal way for opinion mining in highly specific domains. By exploring across a range of techniques and experiments, we find that automated class abstraction approaches in particular the unsupervised approach performs remarkably well against domain expert baseline on text classification tasks. This has the potential to inspire opinion mining applications in order to support market researchers in practice and to inspire fine-grained automated content analysis on a large scale.

==> Conclusion.tex <==
% \subsection{Findings}

% We presented a systematic analysis of 3 class abstraction approaches on the organic datasets for text classification tasks. In accordance with the previously explained results, we answer the research questions from Section \nameref{introduction} as follows:\\

% \subsubsection{RQ1 \rqone} \hfill\\
% \hfill\\ Table \ref{summary} summarizes the classification accuracy of all class abstraction approaches. It can be seen that the domain-expert class abstraction offers moderate performances. The potential reason behind it could be the expert class outliers explained in Subsection \nameref{effects}.\\

% \subsubsection{RQ2 \rqtwo} \hfill\\
% \hfill\\ With the results in Fig. \ref{degree}, we can conclude that degree of class abstraction has more impact on LSI-based than CF-IDF-based class abstraction approaches. We discover that a label-sized degree would be the optimal degree for abstraction. This finding not only minimizes the uncertainty, but also simplifies the research process, and reduces extra fine-tuning efforts. \\

% \subsubsection{RQ3 \rqthree} \hfill\\
% \hfill\\ We demonstrate qualitatively in Table \ref{summary} that our automatic class abstractions are able to improve classification over manual, domain expert-based class abstraction. This analysis provides an example to the market researchers on how to leverage artificial intelligence or rather machine learning and NLP techniques to perform large-scale automated content analysis such as building a category system even without considerable expertise in a domain.\\

% \subsubsection{RQ4 \rqfour} \hfill\\
% \hfill\\ We observe in Table \ref{summary} that our unsupervised class abstraction approach outperforms expert-based class abstraction with margin. It is proved to be able to generate a meaningful intrinsic class hierarchy based on the available data without any human interference. Our finding shows that automated class abstraction can serve as an alternative to a domain-expert class abstraction. We perceive a great potential for it and hope the proposed technique would offer valuable guidance for the market researchers.\\

% \subsubsection{RQ5 \rqfive} \hfill\\
% \hfill\\ As explained in Subsection \nameref{effects}, domain-expert-based class abstraction suffers from minority classes. Those classes which have a low amount of documents are not semantically representative enough in classification. Consequentially, they lead to imbalanced abstract class distributions. Thus, achieving not only a satisfying precision but also a high entropy is a demanding task for class abstraction. Nevertheless, our unsupervised class abstraction approach has overcome this issue and achieves a satisfying result.\\

% \subsubsection{RQ6 \rqsix} \hfill\\
% \hfill\\ As shown in Table \ref{embedding}, sentence-level unsupervised class abstraction is proven to be more efficient than word-level. As possible reasons, we recognize label extraction on word-level to be an extremely challenging task as applying simple max-pooling may lead to over-redundant abstract labels.\\

% \subsubsection{RQ7 \rqseven} \hfill\\
% \hfill\\ Given the classification accuracy, according to Fig. \ref{d_document} and Fig. \ref{k_document}, we discover tf-idf document representation combines well with non-embedding-based class abstraction, while cf-idf document representation is particularly suited for embedding-based class abstraction.

% \subsection{Future work}

% \begin{enumerate}
%   \item Improve label extraction for word-level unsupervised class abstraction approach
%   \item Longformer as classification feature
%   \item Try on a different dataset
% \end{enumerate}


==> Experiments.tex <==
% \label{experiments}

% \subsection{Datasets}
% The effectiveness of our class combination approaches is evaluated on the organic datasets\cite{b1}. The organic datasets are generated aiming at exploring organic food beliefs from consumers. The organic food beliefs are gathered from online comments posted on the forums and discussion boards of news websites from both English and German-speaking countries. These beliefs are further structured into superordinate themes and main themes by domain experts. Besides, the organic datasets are multi-labeled since numerous comments have multiple beliefs according to the research. We choose specifically the domain-specific dataset to research how our approach is able to fulfill the requirement even when there is a lack of data. The statistics of the datasets are summarized in Table \ref{tab1}. 

% \begin{table}[t]
% \caption{Organic datasets statistics}
% \begin{center}
% \setlength\tabcolsep{3.1pt}
% \begin{tabular}{lrrrrr}
% Dataset         & Main themes & Themes & Beliefs & Documents & Sentences \\ \hline
% Organic English  & 4           & 21     & 62      & 1099      & 2275      \\
% Organic German  & 4           & 21     & 60      & 789       & 2334     
% \end{tabular}

% \label{tab1}
% \end{center}
% \end{table}


% \subsection{Preprocessing}

% Preprocessing consists of 5 steps. Sentence segmentation extracts sentences from documents which will be used to create sentence-level embedding for unsupervised approaches. Text cleaning utilizes libraries and regular expressions to filter out URLs, stop words, brackets, quotes, line feeds and blank symbols. Multi-label documents are merged using aggregate and group-by functions in Pandas. Optimal cluster number computation determines the optimal number of clusters for organic datasets using decision criteria such as AIC, BIC scores together with Elbow method. Fine-tuning of GloVe utilizes Mittens package \cite{b2} to fine-tune the GloVe word embedding on the organic dataset. We aimed to research if the domain-specific fine-tuned word embedding would boost the performance of our embedding-based class combination approaches.


% \subsection{Baseline}

% We take the manually annotated labels from domain expert as a baseline and compare them with the abstract label obtained from our semi-automated class combination approach regarding classification performance. The manually annotated label consists of 4 main themes and 21 superordinate themes. Accordingly, we have modified our semi-automated class combination approaches to generate 4 coarse-abstract labels and 21 fine-grained-abstract labels.

% \subsection{Supervised class combination approaches}

% The idea of supervised approach is to perform an intrinsic class hierarchies analysis based on existing expert labels. We aim to achieve automated class abstraction by combining expert labels regarding their semantic similarities. The semantic similarity is measured by applying distance metric on variants of document representations. We investigate if the degree of class abstraction, i.e., latent space dimensionality would relate to classification accuracy when constructing document representations. The dimension of the latent space is chosen between 4, 8, 16, 21, 60, 62, and 100 corresponding to the size of expert labels and the result of the optimal number of clusters analysis. Besides, we research among spacy, fasttext aligned and fine-tuned GloVe pre-trained embeddings on the question of which embedding would deliver the best performance for our embedding-based class combination approaches.

% There are 2 main steps for supervised class combination approaches, namely semantic similarity extraction and class combination using agglomerative hierarchical clustering. Semantic similarity extraction is realized by calculating distances on document representations. Agglomerative hierarchical clustering combines similar classes into new abstract classes based on distance matrices obtained from semantic similarity extraction. The closest clusters indicated by the Euclidean distance will be successively merged until K (4 or 21) clusters are formed. 

% \subsubsection{Semantic similarity extraction}

% \begin{figure}[t]
% \centerline{\includegraphics[width=0.5\textwidth]{LSI.png}}
% \caption{An illustration of SVD truncation for LSI. The SVD process decomposes a term-document matrix A into three matrices: a term-dimension matrix T, a singular-value matrix S, and a document-dimension matrix D, where T, S and D matrices are truncated to k dimensions, i.e., k latent topics. \cite{b3}}
% \label{LSI}
% \end{figure}

% \paragraph{Latent Semantic Indexing}
% LSI\cite{b3} utilizes singular value decomposition (SVD) to reveal latent relationships between documents in a corpus. It yields a low-rank approximation for each document and enables to extract document-document semantic similarity in this low-rank document representation. As illustrated in Fig. \ref{LSI}, SVD decomposes a document-term matrix A into term matrix T, singular value matrix S, and document matrix D, where each matrix will be truncated to k dimensions, i.e., k latent topics. We utilized the document matrix D to construct document representation, in which each document is represented as a linear combination of latent topics. The weights of this combination are taken as the vector representation of the document. 

% \paragraph{Word Movers' Distance}

% \begin{figure}[t]
% \centerline{\includegraphics[width=0.5\textwidth]{WMD.png}}
% \caption{An illustration of the word mover’s distance. All
% non-stop words (bold) of both documents are embedded into a
% word2vec space. The distance between the two documents is the
% minimum cumulative distance that all words in document 1 need
% to travel to exactly match document 2.\cite{b4}}
% \label{WMD}
% \end{figure}

% WMD\cite{b4} is the state-of-the-art semantic distance metric in information retrieval. It is measured by the minimum of the earth mover's distance between each word in two documents in embedding space. If the distance is small, words in two documents are semantically close to each other. As illustrated in Fig. \ref{WMD}, WMD is extremely useful when assessing the semantic similarity between documents with semantically close but syntactically different words.


% \paragraph{CF-IDF}

% \begin{figure}[t]
% \centerline{\includegraphics[width=0.5\textwidth]{BOC.png}}
% \caption{An illustration of bag-of-concepts in embedding space visualized by t-SNE. Concepts are represented as the names of baseball players, the names of soccer players and the names of countries. Semantic similar concepts are located closer to each other, while the semantic dissimilar concepts are located distant from each other. \cite{b5}}
% \label{BOC}
% \end{figure}

% The bag-of-concepts create \textit{concepts} through clustering word vectors in embedding space and uses the frequencies of these concept clusters to represent document vectors\cite{b5}. A \textit{concept} is a set of words, which are semantically related and thus close to each other in embedding space as illustrated in Fig. \ref{BOC}. Each word is associated with one \textit{concept}. Since a document consists of multiple words, it could be regarded as a combination of \textit{concept} frequencies. A document in bag-of-concepts is represented by its CF-IDF score, i.e., the counts of these \textit{concepts} with concept frequency in inverse document frequency weighting scheme. The CF-IDF score reflects the importance of a concept in a document relative to the corpus.

% \subsubsection{Agglomerative hierarchical clustering}

% Agglomerative hierarchical clustering\cite{b6} is an algorithm that groups data points into clusters. We use it to merge our expert labels into abstract labels based on distance matrices. Since agglomerative hierarchical clustering is a bottom-up approach, each expert label is first considered as a single-element cluster. We use the weighted-average linkage criteria (WPGMA), which calculates the intra-cluster distance intuitively as the arithmetic mean when forming new clusters. 

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1\textwidth]{overview.png}
%     \caption{An overview of the experimental design. Abstract labels were extracted using supervised and unsupervised class combination approaches. They will be evaluated in a classification task competing with manually annotated expert label as baseline.}
% \end{figure*}

% \subsection{Unsupervised class combination approaches}

% The idea of unsupervised approach is to create an intrinsic class hierarchy based on the raw organic dataset. In contrast to supervised approach, where we utilize expert labels to generate abstract labels, in unsupervised approach, our machine learning algorithms attempt to find automatically the hidden class structure in data by extracting and analyzing features that capture semantic similarity. The semantic similarity is captured by applying clustering algorithms on document-to-vector representations. We tune the number of clusters k in unsupervised clustering approach to either 4 or 21 corresponding to the size of main themes and superordinate themes from the expert label. It allows us to make a comprehensive comparison of classification performance between labels obtained from the expert-labeled raw dataset, supervised class combination approach, and unsupervised class combination approach.

% There are 3 main steps for unsupervised class combination approaches, namely document-to-vector transformation, clustering, and label extraction. We utilize transfer learning to transform documents into vectors. Instead of learning from scratch, the concept of transfer learning using pre-trained models allows us to leverages previous learning outcomes and adapt them efficiently to solve this new task. We also research which level of language is more suitable for unsupervised class abstraction by applying the document-to-vector transformation on both sentence-level and word-level. Clustering is a machine learning technique that involves grouping a set of data points in such a way that data points in the same group are more similar to each other than those in other groups \cite{b7}. In contrast to the supervised approach, abstract label in unsupervised class abstraction is extracted in a completely unsupervised manner without any human interference.

% \subsubsection{Document-to-vector transformation}

% We perform our document-to-vector transformation based on pre-trained word embedding and pre-trained sentence embedding. Pre-trained word embedding is produced by fasttext aligned word vectors computed on Wikipedia \cite{b8}. The advantage of fasttext aligned word vector is its non-orthogonal linear mapping between representations of words from 44 languages. The alignments are performed with the RCSLS method described in \cite{b9}. Since our organic datasets are bilingual, in order to keep the consistency of word representations, fasttext which provides the state-of-the-art bilingual mapping between two languages is preferred. 

% Pre-trained sentence embedding is produced by the multilingual universal sentence encoder (MUSE)\cite{b10}. It embeds text from 16 languages into a shared semantic embedding space using a multi-task trained dual-encoder that learns tied representations using translation-based bridge tasks \cite{b11}. MUSE provides state-of-the-art document representation that is competitive in multiple cross-lingual retrieval tasks.

% \subsubsection{Clustering}

% After exploring several clustering algorithms, K-means clustering \cite{b12} and Gaussian mixture models (GMM) probabilistic clustering \cite{b13} are chosen as the main clustering algorithms. K-means clustering identifies k number of centroids and allocates every data point to the nearest cluster while keeping the number of centroids as small as possible. The position of centroids is randomly initialized, and then iteratively optimized. 

% While GMM is a probabilistic soft-clustering method, it has uncertainty measurements and probabilities which indicate how likely a data point is associated with a specific cluster. GMM assumes all the data points are generated from a mixture of finite number of Gaussian distributions. Each Gaussian K in the mixture captures similar properties or features of the data points. Regarding clustering performance, based on AIC and BIC scores, GMM with diagonal and full variance matrices have been chosen as the best variants. 

% Besides, we adopt bag-of-concepts which generates its \textit{concepts} through applying hierarchical clustering on word vectors in embedding space as another clustering approach on word-level. Each word is clustered to one \textit{concept}. The number of total concepts is comparable to the parameter K in K-means and GMM clustering algorithms.

% \subsubsection{Label extraction}

% Label extraction has been handled differently in sentence level and word level. At sentence level, each document is first segmented into sentences. After applying clustering algorithms on the sentence embedding, each sentence belongs to one and only one cluster. Therefore, the abstract label of the document is the label combination of its sentences. At word level, after applying clustering algorithms on the word embedding, each word belongs to one and only one cluster. Since a document normally consists of more than one word, each document can be regarded as a combination of word-level clusters. We use max-pooling which calculates the maximum word-level label occurrences of the document to determine its abstract label. If there are equal word-level label occurrences, this document would have a multi-label.

% \subsection{Classification}

% We evaluate the performance of our class combination approach on the organic datasets using the gradient boosting classifier. These data sets can be categorized into two document classification tasks, namely 4-labelled classification, and 21-labelled classification. We use 80\% of the data for training and 20\% for testing. Besides, we apply 8-fold cross-validation, which divides the data into 8 folds and ensures that each fold is used as testing set in evaluation. The mean value of the scores from each iteration of 8-fold cross validation determines the overall performance of the model.

% Since all classification tasks in our experiment are multi-label, exact match, hamming loss, F1 macro, F1 micro, and normalized entropy are the metrics that are used to measure the model performance. Exact match indicates the percentage of samples that have all their labels classified correctly. Hamming loss is the fraction of the wrong labels to the total number of labels. Since it is a loss function, its optimal value is zero and its upper bound is one. F1 score can be interpreted as a weighted average of precision and recall, where an F1 score reaches its best value at 1 and worst value at 0. F1 micro and F1 macro differ from each other on the type of averaging performed on the data. F1 micro calculates metrics globally by counting the total true positives, false negatives, and false positives. On the other hand, F1 micro calculates metrics for each label and finds their unweighted mean \cite{b14}. Entropy is a measure of disorder or uncertainty. In information theory, the entropy of a random variable is the average level of \textit{information}, \textit{surprise}, or \textit{uncertainty} inherent in the variable’s possible outcomes \cite{b15}. Normalization makes the distribution of entropy between 0 and 1, where 1 indicates the most uncertainty and 0 indicates the least uncertainty. Based on the classification performance, we aim to research what are the favorable and unfavorable effects of class abstraction and how do these relate to each other.

% Besides the label difference, we research how do document representation techniques affect the classification by comparing the classification performance using 3 different document representations as feature vectors, namely tf-idf, cf-idf, and Transformers DistilBERT. Document's tf-idf vector representation is a vocabulary-sized tf-idf score matrix. Document's cf-idf vector representation is a concept-sized cf-idf score matrix, where concept size is set default to 100. Document's DistilBERT vector representation is a 768-dimensional contextual embedding based on the [CLS] token from Transformers \cite{b16}. 



==> Introduction.tex <==
\label{introduction}

The rise of social media has enabled and sparked user's desires to share opinions publicly online. The user-generated content often reveals their true beliefs towards a certain aspect of things and therefore worth being researched. Typical application fields are qualitative social studies, e.g., market research, consumer feedback, and political surveys. One of the challenges, however, has been the course of parsing and organizing a large amount of data that is becoming available in the form of natural language into a fine-grained class structure, which provides a more digestible and actionable insight. This is normally achieved by injecting the knowledge from domain experts through annotations. Even so, there is much manual labour and massive associated expenses invested for such content analysis on social media texts.

Most of the cases even if the fine-grained expert annotations are provided, they still have a high resolution on only few data points. This is contrary to the requirements of automated textual analyses, e.g., based on natural language processing and machine learning techniques. Consequently, the question of if and how this data can be effectively leveraged is an interesting and challenging research problem. Once this question is solved, it can be learned how much already existing data could be leveraged to inform automated text-mining based analysis.

One requirement of automated textual analyses is to provide a sufficient number of data points for each class to be able to train classification algorithms. Domain experts, therefore, provide a meaningful hierarchy of classes, such that coarse-grained classes always contain fine-grained classes. This principle we refer to as class abstraction. For example, a coarse-grained class named \textit{product} could contain fine-grained classes such as \textit{safety}, \textit{price}, \textit{healthiness}, \textit{taste}, \textit{quality}, \textit{naturalness}, \textit{availability}, etc. The class \textit{safety} itself could also be a coarse-grained class, which contains further fine-grained classes such as \textit{Products contain chemicals}, \textit{Products contain no or less chemicals compared to conventional products}, \textit{Products are safer and better regulated than conventional products}, \textit{Products are not safe}, etc. As we are interested in optimizing the conditions towards improved classification performance, we see the potential to compare domain-expert-based class abstraction to semi-automated class abstraction approaches.

We aim to prove semi-automated class abstraction approaches could perform as well as domain-expert-based class abstraction in text classification tasks. This would notably reduce human effort, labour cost and increase productivity thus accelerate the research process. Automated approaches also provide consistent results with less variability than humans. Not to mention, how it could reactivate existing meaningful content analyses to provide new insights at little cost. We perceive a great potential in semi-automated class abstraction, especially for large-scale content analysis.

We investigate different class abstraction approaches on the organic dataset for text classification tasks. Class abstraction is achieved by combining many fine-grained classes with few samples to few coarse-grained classes with many samples. This can be achieved manually by a domain expert or automatically by hierarchical clustering based on given fine-grained classes. The generation of fine-grained classes in the first place can also be achieved manually by a domain expert or by unsupervised techniques such as traditional clustering methods, e.g., k-means. During the research, we are interested in the following research questions (RQ):

\def \rqone{How good are domain expert labels for automatic classification?}
\def \rqtwo{How does the degree of class abstraction relate to classification accuracy?}
\def \rqthree{Can automatic class abstraction improve classification over manual, domain expert-based class abstraction?}
\def \rqfour{How does this compare to classes which are generated in a completely unsupervised manner?}
\def \rqfive{What are the favorable and the unfavorable effects of automatic and manual class abstraction and how do these relate to each other?}
\def \rqsix{How do different pre-trained word and sentence embeddings perform for our objectives?}
\def \rqseven{How do different document representation techniques compare regarding classification accuracy?}

\begin{enumerate}[label=RQ\arabic*, leftmargin=8mm]
\setlength\itemsep{0em}
\item \rqone
\item \rqtwo
\item \rqthree
\item \rqfour
\item \rqfive
\end{enumerate}


To solidify our formulated research questions, we think it is helpful to consider the following technical optimization-related questions in depth:

\begin{enumerate}[label=RQ\arabic*, leftmargin=8mm]
\setlength\itemsep{0em}
\setcounter{enumi}{5}
\item \rqsix
\item \rqseven
\end{enumerate}

Our research datasets consist of opinions about organic food and related consumer issues on social media in German-speaking countries and the United States. We analyze the differences regarding classification accuracy using labels generated from domain-expert-based class abstraction and semi-automated class abstraction approaches. Semi-automated class abstraction can be further divided into supervised and unsupervised approaches. In supervised class abstraction approach, we utilize the existing expert labels to form new class hierarchies based on pairwise semantic similarities. Degree of class abstraction, i.e., latent space dimensionality, is a parameter we fine-tune in this process. In unsupervised class abstraction approach, we develop machine learning algorithms that automatically discover the hidden class structure in data using transfer learning and clustering techniques. We evaluate the performance difference between pretrained word and pretrained sentence embedding in the course of label extraction for unsupervised approach. Last but not least, we compare different document representations as features regarding classification accuracy and reveal the best combination of document representations and class abstraction approaches.

Our primary contribution in this paper is a new automated class abstraction approach that is able to create a meaningful intrinsic class hierarchy that outperforms domain-expert-based class abstraction in text classification tasks. Section 4 presents first the experiment dataset and explained why a domain-specific one is preferred. Secondly, it introduces the necessary preprocessing steps. Next, we introduce how to utilize directly the knowledge from domain experts as baseline. Most importantly, we present the concepts of supervised and unsupervised class combination approaches with regard to the question how expert labels could be combined into abstract labels based on latent semantic indexing, word mover's distance and bag-of concepts approaches. Besides, we also bring in the knowledge of how it could be done in a completely unsupervised manner using transfer learning and clustering techniques. Finally, we demonstrate the experimental set up for a multi-label classification task including classifier selection, feature choices, and evaluation metrics. Section 5 presents mainly the results. The main contribution is demonstrated as the classification accuracies between class abstraction approaches. We evaluate qualitatively the effect of degree of class abstraction, favourable and unfavourable effects of class abstraction, as well as how do document representation techniques and pretrained embeddings affect the classification. Section 6 concludes the paper.






==> Results.tex <==
% We summarize the main results in Table \ref{summary}, which shows the best variants of both supervised and unsupervised automatic class abstractions outperform the domain expert-based class abstraction baseline. The performance gain is especially obvious for supervised class abstraction in exact matches, f1 micro and hamming loss, while for unsupervised class abstraction in F1 macro and normalized entropy. In the remainder of this section, we discuss the results of classification regarding the previous research questions in detail.

% \begin{table*}[t]
% \caption{Exact match (Em), hamming loss (Hl), F1 macro (Fma), F1 micro (Fmi) , normalized entropy (Ne) for manual domain-expert class abstraction (baseline), best variants of supervised automatic class abstraction (CA) and best variants of unsupervised automatic class abstraction on 4-labelled and 21-labelled English and German text classification tasks based on TF-IDF document representation.}
% \label{summary}
% \setlength\tabcolsep{7.1pt}
% \begin{tabular}{ccccccccccccccccc}
% \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{Corpus}} & \multicolumn{1}{l|}{\multirow{2}{*}{Labels}} & \multicolumn{5}{c|}{Expert CA} & \multicolumn{5}{c|}{Supervised CA} & \multicolumn{5}{c}{Unsupervised CA} \\
% \multicolumn{1}{c|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{Em} & \multicolumn{1}{l}{Hl} & \multicolumn{1}{l}{Fma} & \multicolumn{1}{l}{Fmi} & \multicolumn{1}{l|}{Ne} & \multicolumn{1}{l}{Em} & \multicolumn{1}{l}{Hl} & \multicolumn{1}{l}{Fma} & \multicolumn{1}{l}{Fmi} & \multicolumn{1}{l|}{Ne} & \multicolumn{1}{l}{Em} & \multicolumn{1}{l}{Hl} & \multicolumn{1}{l}{Fma} & \multicolumn{1}{l}{Fmi} & \multicolumn{1}{l}{Ne} \\ \hline
% \multirow{2}{*}{Organic\_EN} & 4 & 0.39 & 0.20 & 0.48 & 0.54 & 0.92 & \textbf{0.67} & \textbf{0.12} & 0.53 & \textbf{0.76} & 0.62 & 0.45 & 0.16 & \textbf{0.54} & 0.60 & \textbf{0.98} \\
%  & 21 & 0.17 & 0.06 & 0.22 & \textbf{0.33} & 0.85 & \textbf{0.19} & 0.05 & 0.18 & 0.32 & 0.81 & 0.18 & \textbf{0.04} & \textbf{0.28} & 0.31 & \textbf{0.97} \\ \hline
% \multirow{2}{*}{Organic\_DE} & 4 & 0.25 & 0.25 & 0.37 & 0.43 & 0.92 & \textbf{0.75} & \textbf{0.1} & 0.31 & 0.81 & 0.46 & 0.32 & 0.26 & \textbf{0.61} & \textbf{0.70} & \textbf{0.94} \\
%  & 21 & 0.16 & 0.06 & 0.13 & 0.27 & 0.86 & \textbf{0.21} & \textbf{0.05} & 0.13 & \textbf{0.37} & 0.72 & 0.08 & 0.11 & \textbf{0.31} & 0.35 & \textbf{0.98}
% \end{tabular}
% \end{table*}

% \subsection{Degree of class abstraction}
% \label{degree}

% We compare how the degree of class abstraction, i.e. latent space dimensionality would relate to classification accuracy when constructing document representations. Degree of class abstraction involves in our supervised LSI-based and CF-IDF-based class abstractions. We conduct the experiment by choosing the dimension of the latent space between 4, 16, 21, 62, and 100 regarding the organic English dataset.

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.5\textwidth]{Radar_degree.png}}
% \caption{Classification performance regarding degree of class abstraction. Supervised LSI-based and CF-IDF-based class abstractions with different latent space dimensionalities were used to generate abstract labels. Those abstract labels were evaluated in 4-labelled and 21-labelled organic English text classification tasks.}
% \label{degree}
% \end{figure}

% Based on Fig. \ref{degree}, degree of class abstraction has more impact on LSI-based class abstraction than CF-IDF-based class abstraction, especially for 4-labelled classification tasks. Despite dissimilar degrees of class abstraction, CF-IDF-based class abstraction still yields similar results. It is worth point out that the degree 4 and 21 corresponding to the label sizes provide most of the cases the maximum entropy in classification. Besides, they often perform as well as the other degrees in the remaining metrics. Thus, based on our experiment it is recommendable to choose a label-sized degree as the desired degree for abstraction. 

% \subsection{Favourable and unfavorable effects of automatic and manual class abstraction}
% \label{effects}

% We observe in Fig. \ref{sideeffect} that although our supervised WMD-based class abstraction approach provides a high exact match, F1 micro scores, and low hamming loss, but it also suffers from extremely low F1 macro and normalized entropy scores. This is due to imbalanced abstract class distribution resulted from expert class outliers. Expert class outliers are those expert classes that have a low amount of documents thus are not semantically representative for the given class. Since our supervised approach is completely based on existing expert classes, those expert class outliers are inevitable. Despite those obstacles, we still tried to achieve better accuracy with as much higher entropy as possible. Thus, the balance of the trade-off between precision and entropy is an unfavourable effect of class abstraction.

% On the other hand, our unsupervised K-means sentence-level class abstraction approach has overcome this issue and achieves a satisfying result. Its F1 micro, F1 macro, and normalized entropy exceed domain-expert class abstraction with margin, while exact match and hamming loss are almost identical. Besides, it can discover new interesting fine-grained classes such as milk that maybe ignored by domain experts. This result proves the effectiveness of our automatic class abstraction and demonstrates that it could improve classification over manual, domain expert-based class abstraction.

% \begin{figure}[t]
% \centerline{\includegraphics[width=0.5\textwidth]{sideeffects.png}}
% \caption{Classification performance between manual domain-expert class abstraction, supervised fine-tuned Glove embedding WMD class abstraction and unsupervised K-means sentence-level class abstraction on 4-labelled organic English text classification task.}
% \label{sideeffect}
% \end{figure}


% \subsection{Document representation}
% \label{representation}

% According to Fig. \ref{d_document}, document representation greatly affects the classification accuracy using domain-expert class abstraction on 21-labelled organic English text classification tasks. Apart from normalized entropy, tf-idf document representation outperforms both cf-idf and distilbert document representations in the remaining metrics. As for 4-labelled classification tasks, all the document representations yield not too dissimilar results.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1\textwidth]{d_document_representation.png}
%     \caption{Classification performance regarding document representations using domain-expert class abstraction on 4-labelled and 21-labelled organic English text classification tasks.}
%     \label{d_document}
% \end{figure*}

% According to Fig. \ref{k_document}, document representation also greatly affects the classification accuracy using K\_means sentence-level class abstraction on 21-labelled organic English text classification tasks. Cf-idf document representation not only outperforms both tf-idf and distilbert document representations in F1 macro and F1 micro with margin but also performs equally well in the remaining metrics. As for 4-labelled classification tasks, cf-idf document representation also yield a slightly advantage.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1\textwidth]{k_document_representation.png}
%     \caption{Classification performance regarding document representations using K\_means sentence-level class abstraction on 4-labelled and 21-labelled organic English text classification tasks.}
%     \label{k_document}
% \end{figure*}

% Therefore, it is recommendable to use tf-idf document representation for non-embedding-based class abstraction and cf-idf document representation for embedding-based class abstraction in text classification tasks.


% \subsection{Pretrained embeddings}
% \label{pretrainedembeddings}

% We observe pretrained sentence embedding outperforms pretrained word embedding in unsupervised clustering-based class abstraction regarding classification accuracy based on English and German dataset. Table \ref{embedding} shows classification performance of the average of unsupervised sentence-embedding-based class abstraction and the average of unsupervised word-embedding-based class abstraction. The most noticeable advantage of sentence-embedding over word-embedding is its high F1 scores and high normalized entropy, especially for English dataset. Word-embedding-based class abstraction on the contrary suffers from low entropy resulted from imbalanced class distribution due to word-level label extraction. 

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[t]
% \caption{Exact match (Em), hamming loss (Hl), F1 macro (Fma), F1 micro (Fmi), normalized entropy (Ne) for average of sentence-embedding-based unsupervised class abstraction and average of word-embedding-based unsupervised class abstraction on 4-labelled and 21-labelled English and German classification tasks based on cf-idf document representation.}
% \label{embedding}
% \setlength\tabcolsep{2.85pt}
% \begin{tabular}{cccccccccccc}
% \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{Corpus}} & \multicolumn{1}{l|}{\multirow{2}{*}{Labels}} & \multicolumn{5}{c|}{Sent\_Avg} & \multicolumn{5}{c|}{Word\_Avg} \\
% \multicolumn{1}{c|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{Em} & \multicolumn{1}{l}{Hl} & \multicolumn{1}{l}{Fma} & \multicolumn{1}{l}{Fmi} & \multicolumn{1}{l|}{Ne} & \multicolumn{1}{l}{Em} & \multicolumn{1}{l}{Hl} & \multicolumn{1}{l}{Fma} & \multicolumn{1}{l}{Fmi} & \multicolumn{1}{l|}{Ne} \\ \hline
% \multirow{2}{*}{EN} & 4 & 0.39 & 0.21 & \textbf{0.71} & \textbf{0.75} & \textbf{0.97} & \textbf{0.45} & \textbf{0.19} & 0.55 & 0.60 & 0.75 \\
%  & 21 & 0.12 & 0.10 & \textbf{0.40} & \textbf{0.45} & \textbf{0.97} & \textbf{0.22} & \textbf{0.06} & 0.19 & 0.35 & 0.76 \\ \hline
% \multirow{2}{*}{DE} & 4 & 0.1 & 0.44 & \textbf{0.41} & 0.48 & \textbf{0.95} & \textbf{0.61} & \textbf{0.14} & 0.40 & \textbf{0.73} & 0.49 \\
%  & 21 & 0.01 & 0.14 & 0.05 & 0.06 & \textbf{0.97} & \textbf{0.21} & \textbf{0.07} & \textbf{0.19} & \textbf{0.38} & 0.77
% \end{tabular}
% \end{table}






==> Results_new.tex <==

% \subsection{Classification evaluation}

% \subsubsection{Comparison of expert labels and abstract labels}

% \subsubsection{Comparison of supervised and unsupervised class abstraction}

% \subsubsection{Comparison of document feature representation}

% \begin{table*}[t]
% \caption{Supervised abstract label vs. expert label on English organic dataset classification.}
% \label{tab:results_supervised_en}
% \setlength\tabcolsep{2.2pt}
% \begin{tabular}{lcccccccccc}
% \hline
% \multicolumn{1}{c|}{Dataset} & \multicolumn{5}{c|}{ORGANIC\_EN\_4} & \multicolumn{5}{c}{ORGANIC\_EN\_21} \\ \hline
% \multicolumn{1}{c|}{Metrices} & \multicolumn{1}{c|}{Exact match} & \multicolumn{1}{c|}{Hamming loss} & \multicolumn{1}{c|}{F1 macro} & \multicolumn{1}{c|}{F1 micro} & \multicolumn{1}{c|}{Normalized entropy} & \multicolumn{1}{c|}{Exact match} & \multicolumn{1}{c|}{Hamming loss} & \multicolumn{1}{c|}{F1 macro} & \multicolumn{1}{c|}{F1 micro} & Normalized entropy \\ \hline
% \multicolumn{11}{c}{SUPERVISED\_TF\_IDF} \\ \hline
% \multicolumn{1}{l|}{Raw} & \multicolumn{1}{c|}{0.39224} & \multicolumn{1}{c|}{0.20402} & \multicolumn{1}{c|}{0.48797} & \multicolumn{1}{c|}{0.54981} & \multicolumn{1}{c|}{\textbf{0.9270}} & \multicolumn{1}{c|}{0.17385} & \multicolumn{1}{c|}{0.05809} & \multicolumn{1}{c|}{\textbf{0.21756}} & \multicolumn{1}{c|}{0.3341} & 0.8538 \\ \hline
% \multicolumn{1}{l|}{LSI\_4} & \multicolumn{1}{c|}{0.67614} & \multicolumn{1}{c|}{0.12545} & \multicolumn{1}{c|}{\textbf{0.53104}} & \multicolumn{1}{c|}{0.76319} & \multicolumn{1}{c|}{0.6253} & \multicolumn{1}{c|}{0.10444} & \multicolumn{1}{c|}{0.06217} & \multicolumn{1}{c|}{0.1536} & \multicolumn{1}{c|}{0.21082} & 0.8688 \\
% \multicolumn{1}{l|}{LSI\_8} & \multicolumn{1}{c|}{0.8335} & \multicolumn{1}{c|}{0.06172} & \multicolumn{1}{c|}{0.50188} & \multicolumn{1}{c|}{0.88194} & \multicolumn{1}{c|}{0.3773} & \multicolumn{1}{c|}{0.12628} & \multicolumn{1}{c|}{0.06036} & \multicolumn{1}{c|}{0.15785} & \multicolumn{1}{c|}{0.25286} & \textbf{0.8729} \\
% \multicolumn{1}{l|}{LSI\_21} & \multicolumn{1}{c|}{0.85645} & \multicolumn{1}{c|}{0.0557} & \multicolumn{1}{c|}{0.50337} & \multicolumn{1}{c|}{0.89265} & \multicolumn{1}{c|}{0.3465} & \multicolumn{1}{c|}{0.14236} & \multicolumn{1}{c|}{0.05949} & \multicolumn{1}{c|}{0.17591} & \multicolumn{1}{c|}{0.27142} & 0.8621 \\
% \multicolumn{1}{l|}{LSI\_60} & \multicolumn{1}{c|}{0.56941} & \multicolumn{1}{c|}{0.1642} & \multicolumn{1}{c|}{0.40614} & \multicolumn{1}{c|}{0.68674} & \multicolumn{1}{c|}{0.679} & \multicolumn{1}{c|}{0.18945} & \multicolumn{1}{c|}{0.05538} & \multicolumn{1}{c|}{0.17651} & \multicolumn{1}{c|}{0.29832} & 0.8234 \\
% \multicolumn{1}{l|}{LSI\_100} & \multicolumn{1}{c|}{0.74284} & \multicolumn{1}{c|}{0.09787} & \multicolumn{1}{c|}{0.40625} & \multicolumn{1}{c|}{0.81478} & \multicolumn{1}{c|}{0.4781} & \multicolumn{1}{c|}{0.19633} & \multicolumn{1}{c|}{0.05413} & \multicolumn{1}{c|}{0.18563} & \multicolumn{1}{c|}{0.32241} & 0.8122 \\
% \multicolumn{1}{l|}{LSI\_Avg} & \multicolumn{1}{c|}{0.73567} & \multicolumn{1}{c|}{0.10099} & \multicolumn{1}{c|}{0.46974} & \multicolumn{1}{c|}{0.80786} & \multicolumn{1}{c|}{0.50124} & \multicolumn{1}{c|}{0.15177} & \multicolumn{1}{c|}{0.05830} & \multicolumn{1}{c|}{0.1699} & \multicolumn{1}{c|}{0.271167} & 0.84788 \\ \hline
% \multicolumn{1}{l|}{WMD\_spacy} & \multicolumn{1}{c|}{0.92816} & \multicolumn{1}{c|}{0.02658} & \multicolumn{1}{c|}{0.27695} & \multicolumn{1}{c|}{0.94768} & \multicolumn{1}{c|}{0.1331} & \multicolumn{1}{c|}{0.29454} & \multicolumn{1}{c|}{0.05036} & \multicolumn{1}{c|}{0.1218} & \multicolumn{1}{c|}{0.44028} & 0.6203 \\
% \multicolumn{1}{l|}{WMD\_glove} & \multicolumn{1}{c|}{0.89799} & \multicolumn{1}{c|}{0.03987} & \multicolumn{1}{c|}{0.25072} & \multicolumn{1}{c|}{0.92165} & \multicolumn{1}{c|}{0.1945} & \multicolumn{1}{c|}{0.24138} & \multicolumn{1}{c|}{0.05241} & \multicolumn{1}{c|}{0.10107} & \multicolumn{1}{c|}{0.39192} & 0.6151 \\
% \multicolumn{1}{l|}{WMD\_fasttext} & \multicolumn{1}{c|}{0.9454} & \multicolumn{1}{c|}{0.02119} & \multicolumn{1}{c|}{0.24579} & \multicolumn{1}{c|}{0.95802} & \multicolumn{1}{c|}{0.1003} & \multicolumn{1}{c|}{\textbf{0.43678}} & \multicolumn{1}{c|}{\textbf{0.04365}} & \multicolumn{1}{c|}{0.09757} & \multicolumn{1}{c|}{\textbf{0.57799}} & 0.4708 \\
% \multicolumn{1}{l|}{WMD\_Avg} & \multicolumn{1}{c|}{0.92385} & \multicolumn{1}{c|}{0.02921} & \multicolumn{1}{c|}{0.25782} & \multicolumn{1}{c|}{0.94245} & \multicolumn{1}{c|}{0.14263} & \multicolumn{1}{c|}{0.324233} & \multicolumn{1}{c|}{0.048807} & \multicolumn{1}{c|}{0.10681} & \multicolumn{1}{c|}{0.47006} & 0.56873 \\ \hline
% \multicolumn{1}{l|}{CF\_IDF\_4} & \multicolumn{1}{c|}{0.91236} & \multicolumn{1}{c|}{0.03376} & \multicolumn{1}{c|}{0.25029} & \multicolumn{1}{c|}{0.93375} & \multicolumn{1}{c|}{0.1643} & \multicolumn{1}{c|}{0.09195} & \multicolumn{1}{c|}{0.06377} & \multicolumn{1}{c|}{0.09959} & \multicolumn{1}{c|}{0.18388} & 0.7736 \\
% \multicolumn{1}{l|}{CF\_IDF\_8} & \multicolumn{1}{c|}{\textbf{0.96552}} & \multicolumn{1}{c|}{\textbf{0.01473}} & \multicolumn{1}{c|}{0.24671} & \multicolumn{1}{c|}{\textbf{0.97061}} & \multicolumn{1}{c|}{0.0669} & \multicolumn{1}{c|}{0.1681} & \multicolumn{1}{c|}{0.05802} & \multicolumn{1}{c|}{0.12643} & \multicolumn{1}{c|}{0.30163} & 0.7538 \\
% \multicolumn{1}{l|}{CF\_IDF\_21} & \multicolumn{1}{c|}{0.91236} & \multicolumn{1}{c|}{0.03161} & \multicolumn{1}{c|}{0.30029} & \multicolumn{1}{c|}{0.9378} & \multicolumn{1}{c|}{0.1739} & \multicolumn{1}{c|}{0.22414} & \multicolumn{1}{c|}{0.05556} & \multicolumn{1}{c|}{0.13124} & \multicolumn{1}{c|}{0.36749} & 0.6729 \\
% \multicolumn{1}{l|}{CF\_IDF\_60} & \multicolumn{1}{c|}{0.90517} & \multicolumn{1}{c|}{0.03484} & \multicolumn{1}{c|}{0.28893} & \multicolumn{1}{c|}{0.93168} & \multicolumn{1}{c|}{0.1773} & \multicolumn{1}{c|}{0.31897} & \multicolumn{1}{c|}{0.05289} & \multicolumn{1}{c|}{0.17232} & \multicolumn{1}{c|}{0.48913} & 0.6504 \\
% \multicolumn{1}{l|}{CF\_IDF\_100} & \multicolumn{1}{c|}{0.91379} & \multicolumn{1}{c|}{0.03448} & \multicolumn{1}{c|}{0.26087} & \multicolumn{1}{c|}{0.93219} & \multicolumn{1}{c|}{0.16} & \multicolumn{1}{c|}{0.25575} & \multicolumn{1}{c|}{0.0509} & \multicolumn{1}{c|}{0.16341} & \multicolumn{1}{c|}{0.42321} & 0.6598 \\
% \multicolumn{1}{l|}{CF\_IDF\_Avg} & \multicolumn{1}{c|}{0.92184} & \multicolumn{1}{c|}{0.02989} & \multicolumn{1}{c|}{0.26942} & \multicolumn{1}{c|}{0.94121} & \multicolumn{1}{c|}{0.1485} & \multicolumn{1}{c|}{0.21178} & \multicolumn{1}{c|}{0.05623} & \multicolumn{1}{c|}{0.1386} & \multicolumn{1}{c|}{0.3531} & 0.7021 \\ \hline
% \multicolumn{11}{c}{SUPERVISED\_CF\_IDF} \\ \hline
% \multicolumn{1}{l|}{Raw} & \multicolumn{1}{c|}{0.39224} & \multicolumn{1}{c|}{0.22019} & \multicolumn{1}{c|}{0.4717} & \multicolumn{1}{c|}{0.54249} & \multicolumn{1}{c|}{\textbf{0.927}} & \multicolumn{1}{c|}{0.16236} & \multicolumn{1}{c|}{0.06089} & \multicolumn{1}{c|}{0.17881} & \multicolumn{1}{c|}{0.28854} & 0.8538 \\ \hline
% \multicolumn{1}{l|}{LSI\_4} & \multicolumn{1}{c|}{0.6555} & \multicolumn{1}{c|}{0.12804} & \multicolumn{1}{c|}{0.44222} & \multicolumn{1}{c|}{0.75874} & \multicolumn{1}{c|}{0.6253} & \multicolumn{1}{c|}{0.08498} & \multicolumn{1}{c|}{0.0614} & \multicolumn{1}{c|}{0.11998} & \multicolumn{1}{c|}{0.18369} & 0.8688 \\
% \multicolumn{1}{l|}{LSI\_8} & \multicolumn{1}{c|}{0.81285} & \multicolumn{1}{c|}{0.07032} & \multicolumn{1}{c|}{0.41953} & \multicolumn{1}{c|}{0.86518} & \multicolumn{1}{c|}{0.3773} & \multicolumn{1}{c|}{0.1125} & \multicolumn{1}{c|}{0.06222} & \multicolumn{1}{c|}{0.13806} & \multicolumn{1}{c|}{0.22539} & \textbf{0.8729} \\
% \multicolumn{1}{l|}{LSI\_21} & \multicolumn{1}{c|}{0.83464} & \multicolumn{1}{c|}{0.06315} & \multicolumn{1}{c|}{0.42755} & \multicolumn{1}{c|}{0.87891} & \multicolumn{1}{c|}{0.3465} & \multicolumn{1}{c|}{0.10677} & \multicolumn{1}{c|}{0.06331} & \multicolumn{1}{c|}{0.14663} & \multicolumn{1}{c|}{0.22318} & 0.8621 \\
% \multicolumn{1}{l|}{LSI\_60} & \multicolumn{1}{c|}{0.57862} & \multicolumn{1}{c|}{0.15529} & \multicolumn{1}{c|}{0.40715} & \multicolumn{1}{c|}{0.7022} & \multicolumn{1}{c|}{0.679} & \multicolumn{1}{c|}{0.16994} & \multicolumn{1}{c|}{0.0568} & \multicolumn{1}{c|}{0.1536} & \multicolumn{1}{c|}{0.293} & 0.8234 \\
% \multicolumn{1}{l|}{LSI\_100} & \multicolumn{1}{c|}{0.74285} & \multicolumn{1}{c|}{0.10561} & \multicolumn{1}{c|}{0.38857} & \multicolumn{1}{c|}{0.79834,} & \multicolumn{1}{c|}{0.4781} & \multicolumn{1}{c|}{0.17105} & \multicolumn{1}{c|}{0.05647} & \multicolumn{1}{c|}{0.15013} & \multicolumn{1}{c|}{0.3056} & 0.8122 \\
% \multicolumn{1}{l|}{LSI\_Avg} & \multicolumn{1}{c|}{0.72489} & \multicolumn{1}{c|}{0.10448} & \multicolumn{1}{c|}{0.417} & \multicolumn{1}{c|}{0.80126} & \multicolumn{1}{c|}{0.50124} & \multicolumn{1}{c|}{0.12905} & \multicolumn{1}{c|}{0.06004} & \multicolumn{1}{c|}{0.14168} & \multicolumn{1}{c|}{0.24617} & 0.8479 \\ \hline
% \multicolumn{1}{l|}{WMD\_spacy} & \multicolumn{1}{c|}{0.91236} & \multicolumn{1}{c|}{0.03197} & \multicolumn{1}{c|}{0.24464} & \multicolumn{1}{c|}{0.93756} & \multicolumn{1}{c|}{0.1331} & \multicolumn{1}{c|}{0.2931} & \multicolumn{1}{c|}{0.05166} & \multicolumn{1}{c|}{0.12768} & \multicolumn{1}{c|}{0.42815} & 0.6203 \\
% \multicolumn{1}{l|}{WMD\_glove} & \multicolumn{1}{c|}{0.88793} & \multicolumn{1}{c|}{0.04167} & \multicolumn{1}{c|}{0.24161} & \multicolumn{1}{c|}{0.91826} & \multicolumn{1}{c|}{0.1945} & \multicolumn{1}{c|}{0.25431} & \multicolumn{1}{c|}{0.05391} & \multicolumn{1}{c|}{0.10745} & \multicolumn{1}{c|}{0.40397} & 0.6151 \\
% \multicolumn{1}{l|}{WMD\_fasttext} & \multicolumn{1}{c|}{0.94109} & \multicolumn{1}{c|}{0.02191} & \multicolumn{1}{c|}{0.25657} & \multicolumn{1}{c|}{0.95687} & \multicolumn{1}{c|}{0.1003} & \multicolumn{1}{c|}{0.43391} & \multicolumn{1}{c|}{0.04447} & \multicolumn{1}{c|}{0.09499} & \multicolumn{1}{c|}{0.57489} & 0.4708 \\
% \multicolumn{1}{l|}{WMD\_Avg} & \multicolumn{1}{c|}{0.91379} & \multicolumn{1}{c|}{0.03185} & \multicolumn{1}{c|}{0.24761} & \multicolumn{1}{c|}{0.93756} & \multicolumn{1}{c|}{0.14263} & \multicolumn{1}{c|}{0.32711} & \multicolumn{1}{c|}{0.05001} & \multicolumn{1}{c|}{0.11004} & \multicolumn{1}{c|}{0.46900} & 0.5687 \\ \hline
% \multicolumn{1}{l|}{CF\_IDF\_4} & \multicolumn{1}{c|}{0.91954} & \multicolumn{1}{c|}{0.03125} & \multicolumn{1}{c|}{0.25798} & \multicolumn{1}{c|}{0.93873} & \multicolumn{1}{c|}{0.1643} & \multicolumn{1}{c|}{0.0704} & \multicolumn{1}{c|}{0.06637} & \multicolumn{1}{c|}{0.08844} & \multicolumn{1}{c|}{0.15344} & 0.7736 \\
% \multicolumn{1}{l|}{CF\_IDF\_8} & \multicolumn{1}{c|}{0.95546} & \multicolumn{1}{c|}{0.01652} & \multicolumn{1}{c|}{0.24671} & \multicolumn{1}{c|}{0.96725} & \multicolumn{1}{c|}{0.0669} & \multicolumn{1}{c|}{0.17105} & \multicolumn{1}{c|}{0.05647} & \multicolumn{1}{c|}{0.15013} & \multicolumn{1}{c|}{0.3056} & 0.7538 \\
% \multicolumn{1}{l|}{CF\_IDF\_21} & \multicolumn{1}{c|}{0.91954} & \multicolumn{1}{c|}{0.02945} & \multicolumn{1}{c|}{0.28306} & \multicolumn{1}{c|}{0.9423} & \multicolumn{1}{c|}{0.1739} & \multicolumn{1}{c|}{0.23851} & \multicolumn{1}{c|}{0.05658} & \multicolumn{1}{c|}{0.13931} & \multicolumn{1}{c|}{0.4028} & 0.6729 \\
% \multicolumn{1}{l|}{CF\_IDF\_60} & \multicolumn{1}{c|}{0.91379} & \multicolumn{1}{c|}{0.03125} & \multicolumn{1}{c|}{0.29006} & \multicolumn{1}{c|}{0.93872} & \multicolumn{1}{c|}{0.1773} & \multicolumn{1}{c|}{0.3046} & \multicolumn{1}{c|}{0.05549} & \multicolumn{1}{c|}{0.14488} & \multicolumn{1}{c|}{0.46509} & 0.6504 \\
% \multicolumn{1}{l|}{CF\_IDF\_100} & \multicolumn{1}{c|}{0.89943} & \multicolumn{1}{c|}{0.03807} & \multicolumn{1}{c|}{0.25435} & \multicolumn{1}{c|}{0.92583} & \multicolumn{1}{c|}{0.16} & \multicolumn{1}{c|}{0.24856} & \multicolumn{1}{c|}{0.05432} & \multicolumn{1}{c|}{0.14913} & \multicolumn{1}{c|}{0.42919} & 0.6598 \\
% \multicolumn{1}{l|}{CF\_IDF\_Avg} & \multicolumn{1}{c|}{0.92155} & \multicolumn{1}{c|}{0.02931} & \multicolumn{1}{c|}{0.26643} & \multicolumn{1}{c|}{0.94257} & \multicolumn{1}{c|}{0.1485} & \multicolumn{1}{c|}{0.20662} & \multicolumn{1}{c|}{0.05785} & \multicolumn{1}{c|}{0.13438} & \multicolumn{1}{c|}{0.35122} & 0.7021 \\ \hline
% \multicolumn{11}{c}{SUPERVISED\_DISTILBERT} \\ \hline
% \multicolumn{1}{l|}{Raw} & \multicolumn{1}{c|}{0.41379} & \multicolumn{1}{c|}{0.2069} & \multicolumn{1}{c|}{0.46427} & \multicolumn{1}{c|}{0.55995} & \multicolumn{1}{c|}{\textbf{0.927}} & \multicolumn{1}{c|}{0.08333} & \multicolumn{1}{c|}{0.06527} & \multicolumn{1}{c|}{0.10169} & \multicolumn{1}{c|}{0.19156} & 0.8538 \\ \hline
% \multicolumn{1}{l|}{LSI\_4} & \multicolumn{1}{c|}{0.6498} & \multicolumn{1}{c|}{0.13262} & \multicolumn{1}{c|}{0.39465} & \multicolumn{1}{c|}{0.74389} & \multicolumn{1}{c|}{0.6253} & \multicolumn{1}{c|}{0.07348} & \multicolumn{1}{c|}{0.06588} & \multicolumn{1}{c|}{0.09586} & \multicolumn{1}{c|}{0.16842} & 0.8688 \\
% \multicolumn{1}{l|}{LSI\_8} & \multicolumn{1}{c|}{0.80252} & \multicolumn{1}{c|}{0.07835} & \multicolumn{1}{c|}{0.33368} & \multicolumn{1}{c|}{0.84834} & \multicolumn{1}{c|}{0.3773} & \multicolumn{1}{c|}{0.07002} & \multicolumn{1}{c|}{0.06299} & \multicolumn{1}{c|}{0.10533} & \multicolumn{1}{c|}{0.17235} & \textbf{0.8729} \\
% \multicolumn{1}{l|}{LSI\_21} & \multicolumn{1}{c|}{0.8312} & \multicolumn{1}{c|}{0.0666} & \multicolumn{1}{c|}{0.35693} & \multicolumn{1}{c|}{0.87052} & \multicolumn{1}{c|}{0.3465} & \multicolumn{1}{c|}{0.06889} & \multicolumn{1}{c|}{0.06288} & \multicolumn{1}{c|}{0.10109} & \multicolumn{1}{c|}{0.17185} & 0.8621 \\
% \multicolumn{1}{l|}{LSI\_60} & \multicolumn{1}{c|}{0.58204} & \multicolumn{1}{c|}{0.15243} & \multicolumn{1}{c|}{0.38709} & \multicolumn{1}{c|}{0.70717} & \multicolumn{1}{c|}{0.679} & \multicolumn{1}{c|}{0.13086} & \multicolumn{1}{c|}{0.05905} & \multicolumn{1}{c|}{0.10742} & \multicolumn{1}{c|}{0.23889} & 0.8234 \\
% \multicolumn{1}{l|}{LSI\_100} & \multicolumn{1}{c|}{0.74857} & \multicolumn{1}{c|}{0.09442} & \multicolumn{1}{c|}{0.36401} & \multicolumn{1}{c|}{0.81748} & \multicolumn{1}{c|}{0.4781} & \multicolumn{1}{c|}{0.14009} & \multicolumn{1}{c|}{0.05812} & \multicolumn{1}{c|}{0.11212} & \multicolumn{1}{c|}{0.26609} & 0.8122 \\
% \multicolumn{1}{l|}{LSI\_Avg} & \multicolumn{1}{c|}{0.72283} & \multicolumn{1}{c|}{0.10488} & \multicolumn{1}{c|}{0.36727} & \multicolumn{1}{c|}{0.79748} & \multicolumn{1}{c|}{0.50124} & \multicolumn{1}{c|}{0.09667} & \multicolumn{1}{c|}{0.061784} & \multicolumn{1}{c|}{0.10436} & \multicolumn{1}{c|}{0.20352} & 0.84788 \\ \hline
% \multicolumn{1}{l|}{WMD\_spacy} & \multicolumn{1}{c|}{0.9296} & \multicolumn{1}{c|}{0.0273} & \multicolumn{1}{c|}{0.29636} & \multicolumn{1}{c|}{0.94604} & \multicolumn{1}{c|}{0.1331} & \multicolumn{1}{c|}{0.25718} & \multicolumn{1}{c|}{0.05343} & \multicolumn{1}{c|}{0.09362} & \multicolumn{1}{c|}{0.39947} & 0.6203 \\
% \multicolumn{1}{l|}{WMD\_glove} & \multicolumn{1}{c|}{0.89368} & \multicolumn{1}{c|}{0.04023} & \multicolumn{1}{c|}{0.25372} & \multicolumn{1}{c|}{0.92079} & \multicolumn{1}{c|}{0.1945} & \multicolumn{1}{c|}{0.22414} & \multicolumn{1}{c|}{0.05364} & \multicolumn{1}{c|}{0.08803} & \multicolumn{1}{c|}{0.36481} & 0.6151 \\
% \multicolumn{1}{l|}{WMD\_fasttext} & \multicolumn{1}{c|}{0.94684} & \multicolumn{1}{c|}{0.02083} & \multicolumn{1}{c|}{0.256} & \multicolumn{1}{c|}{0.95863} & \multicolumn{1}{c|}{0.1003} & \multicolumn{1}{c|}{0.42529} & \multicolumn{1}{c|}{0.04495} & \multicolumn{1}{c|}{0.08752} & \multicolumn{1}{c|}{0.56297} & 0.4708 \\
% \multicolumn{1}{l|}{WMD\_Avg} & \multicolumn{1}{c|}{0.92337} & \multicolumn{1}{c|}{0.02945} & \multicolumn{1}{c|}{0.26869} & \multicolumn{1}{c|}{0.94182} & \multicolumn{1}{c|}{0.14263} & \multicolumn{1}{c|}{0.30220} & \multicolumn{1}{c|}{0.05067} & \multicolumn{1}{c|}{0.08972} & \multicolumn{1}{c|}{0.44241} & 0.56873 \\ \hline
% \multicolumn{1}{l|}{CF\_IDF\_4} & \multicolumn{1}{c|}{0.90661} & \multicolumn{1}{c|}{0.03556} & \multicolumn{1}{c|}{0.26005} & \multicolumn{1}{c|}{0.92985} & \multicolumn{1}{c|}{0.1643} & \multicolumn{1}{c|}{0.06178} & \multicolumn{1}{c|}{0.06698} & \multicolumn{1}{c|}{0.07666} & \multicolumn{1}{c|}{0.16427} & 0.7736 \\
% \multicolumn{1}{l|}{CF\_IDF\_8} & \multicolumn{1}{c|}{0.96408} & \multicolumn{1}{c|}{0.01509} & \multicolumn{1}{c|}{0.26944} & \multicolumn{1}{c|}{0.96996} & \multicolumn{1}{c|}{0.0669} & \multicolumn{1}{c|}{0.17098} & \multicolumn{1}{c|}{0.05966} & \multicolumn{1}{c|}{0.12527} & \multicolumn{1}{c|}{0.31208} & 0.7538 \\
% \multicolumn{1}{l|}{CF\_IDF\_21} & \multicolumn{1}{c|}{0.90661} & \multicolumn{1}{c|}{0.03448} & \multicolumn{1}{c|}{0.28111} & \multicolumn{1}{c|}{0.93198} & \multicolumn{1}{c|}{0.1739} & \multicolumn{1}{c|}{0.19828} & \multicolumn{1}{c|}{0.05946} & \multicolumn{1}{c|}{0.10286} & \multicolumn{1}{c|}{0.34426} & 0.6729 \\
% \multicolumn{1}{l|}{CF\_IDF\_60} & \multicolumn{1}{c|}{0.90374} & \multicolumn{1}{c|}{0.03628} & \multicolumn{1}{c|}{0.26773} & \multicolumn{1}{c|}{0.92866} & \multicolumn{1}{c|}{0.1773} & \multicolumn{1}{c|}{0.25862} & \multicolumn{1}{c|}{0.0585} & \multicolumn{1}{c|}{0.09714} & \multicolumn{1}{c|}{0.41884} & 0.6504 \\
% \multicolumn{1}{l|}{CF\_IDF\_100} & \multicolumn{1}{c|}{0.90661} & \multicolumn{1}{c|}{0.03592} & \multicolumn{1}{c|}{0.26085} & \multicolumn{1}{c|}{0.92916} & \multicolumn{1}{c|}{0.16} & \multicolumn{1}{c|}{0.22701} & \multicolumn{1}{c|}{0.05638} & \multicolumn{1}{c|}{0.10805} & \multicolumn{1}{c|}{0.37226} & 0.6598 \\
% \multicolumn{1}{l|}{CF\_IDF\_Avg} & \multicolumn{1}{c|}{0.91753} & \multicolumn{1}{c|}{0.03147} & \multicolumn{1}{c|}{0.26784} & \multicolumn{1}{c|}{0.93792} & \multicolumn{1}{c|}{0.14848} & \multicolumn{1}{c|}{0.18333} & \multicolumn{1}{c|}{0.06019} & \multicolumn{1}{c|}{0.10199} & \multicolumn{1}{c|}{0.32234} & 0.7021 \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[t]
% \caption{Unsupervised abstract label vs. expert label on English organic dataset classification.}
% \label{tab:results_unsupervised_en}
% \setlength\tabcolsep{2.2pt}
% \begin{tabular}{lcccccccccc}
% \hline
% \multicolumn{1}{c|}{Dataset} & \multicolumn{5}{c|}{ORGANIC\_EN\_4} & \multicolumn{5}{c}{ORGANIC\_EN\_21} \\ \hline
% \multicolumn{1}{c|}{Metrices} & \multicolumn{1}{c|}{Exact match} & \multicolumn{1}{c|}{Hamming loss} & \multicolumn{1}{c|}{F1 macro} & \multicolumn{1}{c|}{F1 micro} & \multicolumn{1}{c|}{Normalized entropy} & \multicolumn{1}{c|}{Exact match} & \multicolumn{1}{c|}{Hamming loss} & \multicolumn{1}{c|}{F1 macro} & \multicolumn{1}{c|}{F1 micro} & Normalized entropy \\ \hline
% \multicolumn{11}{c}{UNSUPERVISED\_TF\_IDF} \\ \hline
% \multicolumn{1}{l|}{Raw} & \multicolumn{1}{c|}{0.39224} & \multicolumn{1}{c|}{0.20402} & \multicolumn{1}{c|}{0.48797} & \multicolumn{1}{c|}{0.54981} & \multicolumn{1}{c|}{0.927} & \multicolumn{1}{c|}{0.17385} & \multicolumn{1}{c|}{0.05809} & \multicolumn{1}{c|}{0.21756} & \multicolumn{1}{c|}{0.3341} & 0.8538 \\ \hline
% \multicolumn{1}{l|}{Sent\_K\_means} & \multicolumn{1}{c|}{0.38218} & \multicolumn{1}{c|}{0.22593} & \multicolumn{1}{c|}{0.67418} & \multicolumn{1}{c|}{0.72276} & \multicolumn{1}{c|}{0.9803} & \multicolumn{1}{c|}{0.10632} & \multicolumn{1}{c|}{0.10352} & \multicolumn{1}{c|}{0.33343} & \multicolumn{1}{c|}{0.38341} & 0.9582 \\
% \multicolumn{1}{l|}{Sent\_GMM\_diag} & \multicolumn{1}{c|}{0.37787} & \multicolumn{1}{c|}{0.23348} & \multicolumn{1}{c|}{0.68768} & \multicolumn{1}{c|}{0.73332} & \multicolumn{1}{c|}{0.9635} & \multicolumn{1}{c|}{0.10345} & \multicolumn{1}{c|}{0.10324} & \multicolumn{1}{c|}{0.33153} & \multicolumn{1}{c|}{0.37415} & 0.9774 \\
% \multicolumn{1}{l|}{Sent\_GMM\_full} & \multicolumn{1}{c|}{0.37787} & \multicolumn{1}{c|}{0.23671} & \multicolumn{1}{c|}{0.64621} & \multicolumn{1}{c|}{0.70931} & \multicolumn{1}{c|}{0.9739} & \multicolumn{1}{c|}{0.10632} & \multicolumn{1}{c|}{0.10632} & \multicolumn{1}{c|}{0.33029} & \multicolumn{1}{c|}{0.36743} & 0.9797 \\
% \multicolumn{1}{l|}{Sent\_Avg} & \multicolumn{1}{c|}{0.37932} & \multicolumn{1}{c|}{0.23201} & \multicolumn{1}{c|}{0.66932} & \multicolumn{1}{c|}{0.72179} & \multicolumn{1}{c|}{0.9725} & \multicolumn{1}{c|}{0.10531} & \multicolumn{1}{c|}{0.10432} & \multicolumn{1}{c|}{0.33173} & \multicolumn{1}{c|}{0.37491} & 0.9717 \\ \hline
% \multicolumn{1}{l|}{Word\_K\_means} & \multicolumn{1}{c|}{0.28879} & \multicolumn{1}{c|}{0.24138} & \multicolumn{1}{c|}{0.41794} & \multicolumn{1}{c|}{0.46093} & \multicolumn{1}{c|}{0.7078} & \multicolumn{1}{c|}{0.16092} & \multicolumn{1}{c|}{0.07191} & \multicolumn{1}{c|}{0.19693} & \multicolumn{1}{c|}{0.31018} & 0.715 \\
% \multicolumn{1}{l|}{Word\_GMM\_diag} & \multicolumn{1}{c|}{0.32759} & \multicolumn{1}{c|}{0.23815} & \multicolumn{1}{c|}{0.44334} & \multicolumn{1}{c|}{0.50462} & \multicolumn{1}{c|}{0.6856} & \multicolumn{1}{c|}{0.12069} & \multicolumn{1}{c|}{0.07485} & \multicolumn{1}{c|}{0.18467} & \multicolumn{1}{c|}{0.26173} & 0.7397 \\
% \multicolumn{1}{l|}{Word\_GMM\_full} & \multicolumn{1}{c|}{0.27874} & \multicolumn{1}{c|}{0.24713} & \multicolumn{1}{c|}{0.40356} & \multicolumn{1}{c|}{0.44413} & \multicolumn{1}{c|}{0.6998} & \multicolumn{1}{c|}{0.1408} & \multicolumn{1}{c|}{0.07533} & \multicolumn{1}{c|}{0.16635} & \multicolumn{1}{c|}{0.28667} & 0.7396 \\
% \multicolumn{1}{l|}{Word\_CF\_IDF} & \multicolumn{1}{c|}{0.32615} & \multicolumn{1}{c|}{0.30999} & \multicolumn{1}{c|}{0.65348} & \multicolumn{1}{c|}{0.69346} & \multicolumn{1}{c|}{0.9379} & \multicolumn{1}{c|}{0.15086} & \multicolumn{1}{c|}{0.04871} & \multicolumn{1}{c|}{0.11617} & \multicolumn{1}{c|}{0.2481} & 0.8382 \\
% \multicolumn{1}{l|}{Word\_Avg} & \multicolumn{1}{c|}{0.30532} & \multicolumn{1}{c|}{0.25916} & \multicolumn{1}{c|}{0.47958} & \multicolumn{1}{c|}{0.52579} & \multicolumn{1}{c|}{0.7578} & \multicolumn{1}{c|}{0.14331} & \multicolumn{1}{c|}{0.0677} & \multicolumn{1}{c|}{0.16603} & \multicolumn{1}{c|}{0.27667} & 0.75813 \\ \hline
% \multicolumn{11}{c}{UNSUPERVISED\_CF\_IDF} \\ \hline
% \multicolumn{1}{l|}{Raw} & \multicolumn{1}{c|}{0.39224} & \multicolumn{1}{c|}{0.20402} & \multicolumn{1}{c|}{0.48797} & \multicolumn{1}{c|}{0.54981} & \multicolumn{1}{c|}{0.927} & \multicolumn{1}{c|}{0.16236} & \multicolumn{1}{c|}{0.06089} & \multicolumn{1}{c|}{0.17881} & \multicolumn{1}{c|}{0.28854} & 0.8538 \\ \hline
% \multicolumn{1}{l|}{Sent\_K\_means} & \multicolumn{1}{c|}{0.40374} & \multicolumn{1}{c|}{0.20474} & \multicolumn{1}{c|}{0.72276} & \multicolumn{1}{c|}{0.75873} & \multicolumn{1}{c|}{\textbf{0.9822}} & \multicolumn{1}{c|}{0.10201} & \multicolumn{1}{c|}{0.10215} & \multicolumn{1}{c|}{\textbf{0.40939}} & \multicolumn{1}{c|}{0.4401} & 0.9728 \\
% \multicolumn{1}{l|}{Sent\_GMM\_diag} & \multicolumn{1}{c|}{0.3592} & \multicolumn{1}{c|}{0.22845} & \multicolumn{1}{c|}{0.71138} & \multicolumn{1}{c|}{0.73982} & \multicolumn{1}{c|}{0.9706} & \multicolumn{1}{c|}{0.10489} & \multicolumn{1}{c|}{0.10331} & \multicolumn{1}{c|}{0.39693} & \multicolumn{1}{c|}{0.42771} & \textbf{0.9864} \\
% \multicolumn{1}{l|}{Sent\_GMM\_full} & \multicolumn{1}{c|}{0.4296} & \multicolumn{1}{c|}{0.19864} & \multicolumn{1}{c|}{0.70403} & \multicolumn{1}{c|}{\textbf{0.76279}} & \multicolumn{1}{c|}{0.9661} & \multicolumn{1}{c|}{0.1408} & \multicolumn{1}{c|}{0.09996} & \multicolumn{1}{c|}{0.40662} & \multicolumn{1}{c|}{\textbf{0.47662}} & 0.958 \\
% \multicolumn{1}{l|}{Sent\_Avg} & \multicolumn{1}{c|}{0.3975} & \multicolumn{1}{c|}{0.21061} & \multicolumn{1}{c|}{0.71272} & \multicolumn{1}{c|}{0.75378} & \multicolumn{1}{c|}{0.97296} & \multicolumn{1}{c|}{0.1159} & \multicolumn{1}{c|}{0.10180} & \multicolumn{1}{c|}{0.40431} & \multicolumn{1}{c|}{0.44814} & 0.9724 \\ \hline
% \multicolumn{1}{l|}{Word\_K\_means} & \multicolumn{1}{c|}{0.44109} & \multicolumn{1}{c|}{0.19612} & \multicolumn{1}{c|}{0.57192} & \multicolumn{1}{c|}{0.60917} & \multicolumn{1}{c|}{0.7078} & \multicolumn{1}{c|}{0.23132} & \multicolumn{1}{c|}{0.07081} & \multicolumn{1}{c|}{0.20112} & \multicolumn{1}{c|}{0.36259} & 0.715 \\
% \multicolumn{1}{l|}{Word\_GMM\_diag} & \multicolumn{1}{c|}{\textbf{0.48132}} & \multicolumn{1}{c|}{0.18642} & \multicolumn{1}{c|}{0.55261} & \multicolumn{1}{c|}{0.6341} & \multicolumn{1}{c|}{0.6856} & \multicolumn{1}{c|}{0.21264} & \multicolumn{1}{c|}{0.0689} & \multicolumn{1}{c|}{0.19403} & \multicolumn{1}{c|}{0.36119} & 0.7397 \\
% \multicolumn{1}{l|}{Word\_GMM\_full} & \multicolumn{1}{c|}{0.43966} & \multicolumn{1}{c|}{0.20043} & \multicolumn{1}{c|}{0.5642} & \multicolumn{1}{c|}{0.5965} & \multicolumn{1}{c|}{0.6998} & \multicolumn{1}{c|}{\textbf{0.23563}} & \multicolumn{1}{c|}{0.06842} & \multicolumn{1}{c|}{0.22537} & \multicolumn{1}{c|}{0.38593} & 0.7396 \\
% \multicolumn{1}{l|}{Word\_CF\_IDF} & \multicolumn{1}{c|}{0.4181} & \multicolumn{1}{c|}{\textbf{0.17708}} & \multicolumn{1}{c|}{0.51219} & \multicolumn{1}{c|}{0.56706} & \multicolumn{1}{c|}{0.9379} & \multicolumn{1}{c|}{0.19971} & \multicolumn{1}{c|}{\textbf{0.04803}} & \multicolumn{1}{c|}{0.14349} & \multicolumn{1}{c|}{0.32483} & 0.8382 \\
% \multicolumn{1}{l|}{Word\_Avg} & \multicolumn{1}{c|}{0.44504} & \multicolumn{1}{c|}{0.19001} & \multicolumn{1}{c|}{0.55023} & \multicolumn{1}{c|}{0.60171} & \multicolumn{1}{c|}{0.7578} & \multicolumn{1}{c|}{0.21983} & \multicolumn{1}{c|}{0.06404} & \multicolumn{1}{c|}{0.19100} & \multicolumn{1}{c|}{0.35864} & 0.75813 \\ \hline
% \multicolumn{11}{c}{UNSUPERVISED\_DISTILBERT} \\ \hline
% \multicolumn{1}{l|}{Raw} & \multicolumn{1}{c|}{0.41379} & \multicolumn{1}{c|}{0.2069} & \multicolumn{1}{c|}{0.46427} & \multicolumn{1}{c|}{0.55995} & \multicolumn{1}{c|}{0.927} & \multicolumn{1}{c|}{0.08333} & \multicolumn{1}{c|}{0.06527} & \multicolumn{1}{c|}{0.10169} & \multicolumn{1}{c|}{0.19156} & 0.8538 \\ \hline
% \multicolumn{1}{l|}{Sent\_K\_means} & \multicolumn{1}{c|}{0.39511} & \multicolumn{1}{c|}{0.21372} & \multicolumn{1}{c|}{0.72455} & \multicolumn{1}{c|}{0.75171} & \multicolumn{1}{c|}{0.9806} & \multicolumn{1}{c|}{0.10776} & \multicolumn{1}{c|}{0.10516} & \multicolumn{1}{c|}{0.28362} & \multicolumn{1}{c|}{0.34819} & 0.9728 \\
% \multicolumn{1}{l|}{Sent\_GMM\_diag} & \multicolumn{1}{c|}{0.35057} & \multicolumn{1}{c|}{0.22773} & \multicolumn{1}{c|}{\textbf{0.72607}} & \multicolumn{1}{c|}{0.74188} & \multicolumn{1}{c|}{0.9706} & \multicolumn{1}{c|}{0.10776} & \multicolumn{1}{c|}{0.10632} & \multicolumn{1}{c|}{0.28741} & \multicolumn{1}{c|}{0.33812} & 0.9806 \\
% \multicolumn{1}{l|}{Sent\_GMM\_full} & \multicolumn{1}{c|}{0.41667} & \multicolumn{1}{c|}{0.20941} & \multicolumn{1}{c|}{0.70315} & \multicolumn{1}{c|}{0.75484} & \multicolumn{1}{c|}{0.9663} & \multicolumn{1}{c|}{0.10489} & \multicolumn{1}{c|}{0.10584} & \multicolumn{1}{c|}{0.26273} & \multicolumn{1}{c|}{0.3402} & 0.9718 \\
% \multicolumn{1}{l|}{Sent\_Avg} & \multicolumn{1}{c|}{0.38745} & \multicolumn{1}{c|}{0.21695} & \multicolumn{1}{c|}{0.71792} & \multicolumn{1}{c|}{0.74947} & \multicolumn{1}{c|}{0.9725} & \multicolumn{1}{c|}{0.10680} & \multicolumn{1}{c|}{0.10577} & \multicolumn{1}{c|}{0.27792} & \multicolumn{1}{c|}{0.34217} & 0.97506 \\ \hline
% \multicolumn{1}{l|}{Word\_K\_means} & \multicolumn{1}{c|}{0.36782} & \multicolumn{1}{c|}{0.2245} & \multicolumn{1}{c|}{0.50091} & \multicolumn{1}{c|}{0.54283} & \multicolumn{1}{c|}{0.7078} & \multicolumn{1}{c|}{0.10489} & \multicolumn{1}{c|}{0.08108} & \multicolumn{1}{c|}{0.11997} & \multicolumn{1}{c|}{0.21008} & 0.715 \\
% \multicolumn{1}{l|}{Word\_GMM\_diag} & \multicolumn{1}{c|}{0.44684} & \multicolumn{1}{c|}{0.20833} & \multicolumn{1}{c|}{0.50367} & \multicolumn{1}{c|}{0.59975} & \multicolumn{1}{c|}{0.6856} & \multicolumn{1}{c|}{0.13075} & \multicolumn{1}{c|}{0.07807} & \multicolumn{1}{c|}{0.11973} & \multicolumn{1}{c|}{0.22971} & 0.7397 \\
% \multicolumn{1}{l|}{Word\_GMM\_full} & \multicolumn{1}{c|}{0.37787} & \multicolumn{1}{c|}{0.2227} & \multicolumn{1}{c|}{0.49297} & \multicolumn{1}{c|}{0.53855} & \multicolumn{1}{c|}{0.6998} & \multicolumn{1}{c|}{0.12069} & \multicolumn{1}{c|}{0.07861} & \multicolumn{1}{c|}{0.1023} & \multicolumn{1}{c|}{0.22972} & 0.7396 \\
% \multicolumn{1}{l|}{Word\_CF\_IDF} & \multicolumn{1}{c|}{0.37069} & \multicolumn{1}{c|}{0.20402} & \multicolumn{1}{c|}{0.43514} & \multicolumn{1}{c|}{0.49159} & \multicolumn{1}{c|}{0.9379} & \multicolumn{1}{c|}{0.10345} & \multicolumn{1}{c|}{0.05398} & \multicolumn{1}{c|}{0.09344} & \multicolumn{1}{c|}{0.19701} & 0.8382 \\
% \multicolumn{1}{l|}{Word\_Avg} & \multicolumn{1}{c|}{0.39081} & \multicolumn{1}{c|}{0.214888} & \multicolumn{1}{c|}{0.483173} & \multicolumn{1}{c|}{0.54318} & \multicolumn{1}{c|}{0.75778} & \multicolumn{1}{c|}{0.11495} & \multicolumn{1}{c|}{0.07294} & \multicolumn{1}{c|}{0.10886} & \multicolumn{1}{c|}{0.21663} & 0.75813 \\ \hline
% \end{tabular}
% \end{table*}


